Tail Modulo Cons, OCaml, and Relational Separation Logic

Common functional languages incentivize tail-recursive functions, as opposed to general recursive functions that consume stack space and may not scale to large inputs. This distinction occasionally requires writing functions in a tail-recursive style that may be more complex and slower than the natural, non-tail-recursive definition. This work describes our implementation of the *tail modulo constructor* (TMC) transformation in the OCaml compiler, an optimization that provides stack-efficiency for a larger class of functions -- tail-recursive *modulo constructors* -- which includes in particular the natural definition of `List.map` and many similar recursive data-constructing functions. We prove the correctness of this program transformation in a simplified setting -- a small untyped calculus -- that captures the salient aspects of the OCaml implementation. Our proof is mechanized in the Coq proof assistant, using the Iris base logic. An independent contribution of our work is an extension of the Simuliris approach to define simulation relations that support different calling conventions. To our knowledge, this is the first use of Simuliris to prove the correctness of a compiler transformation.

==> conclusion.tex <==
\section{Conclusion and Future Work}

concurrency

effect handlers

compression of constructors

prove other program transformation using this framework (CPS)

% To give another example of simulation with a different protocol,
% we could look at accumulator-passing-style transformations
% (tail-modulo-context for associative arithmetic operators). Prove
% that `factorial` is equivalent to the tmc-optimized factorial
% (two versions, one in accumulator-passing-style and the "direct
% style" version that calls it with accumulator 1).
%    .. et donc il faut garder les entiers!
%
% Clément: j'ai commencé à bosser sur ça. Ça demande de travailler
% sur des expressions plutôt que des valeurs (l'accumulateur peut
% être un entier mais aussi une variable). Il faut regénéraliser
% des bouts du développment Coq qui était spécialisé aux
% valeurs. Il se passe un truc intéressant sur les échecs si
% l'accumulateur est une variable qui est substituée par un
% non-entier (échec pendant le calcul d'un côté, après le calcul
% de l'autre).
% La formulation où on accumule des opérations sur des expressions
% arbitraires et pas juste des constantes entières est un peu plus
% générale que celle de Daan Leijen (que des constantes). Elle permet
% de faire une transformation APS sur List.sum.

==> figures/map_tmc.tex <==
\begin{figure}[tp]
\begin{minipage}{.40\columnwidth}
\begin{Datalang}
map |-> rec (fn, xs) =
  match xs with
  | [] ->
      []
  | x :: xs ->
      let y = fn x in
      let dst = y :: ? in
      @map_dps ((dst, 2), fn, xs) ;
      dst
\end{Datalang}
\end{minipage}
\hfill
\begin{minipage}{.52\columnwidth}
\begin{Datalang}
map_dps |-> rec ((dst, idx), fn, xs) =
  match xs with
  | [] ->
      dst.(idx) <- []
  | x :: xs ->
      let y = fn x in
      let dst' = y :: ? in
      dst.(idx) <- dst' ;
      @map_dps ((dst', 2), fn, xs)
\end{Datalang}
\end{minipage}
\caption{Direct and DPS transforms of \datalang|map| (\cref{fig:map})}
\label{fig:map_tmc}
\end{figure}
